WiPIN: Operation-free Passive Person Identification Using Wi-Fi Signals

Wi-Fi signals-based person identification attracts increasing attention in the booming Internet-of-Things era mainly due to its pervasiveness and passiveness. Most previous work applies gaits extracted from WiFi distortions caused by the person walking to achieve the identification. However, to extract useful gait, a person must walk along a pre-defined path for several meters, which requires user high collaboration and increases identification time overhead, thus limiting use scenarios. Moreover, gait based work has severe shortcoming in identification performance, especially when the user volume is large. In order to eliminate the above limitations, in this paper, we present an operation-free person identification system, namely WiPIN, that requires least user collaboration and achieves good performance. WiPIN is based on an entirely new insight that Wi-Fi signals would carry person body information when propagating through the body, which is potentially discriminated for person identification. Then we demonstrate the feasibility on commodity off-the-shelf Wi-Fi devices by well-designed signal pre-processing, feature extraction, and identity matching algorithms. Results show that WiPIN achieves 92% identification accuracy over 30 users, high robustness to various experimental settings, and low identifying time overhead, i.e., less than 300ms.

==> tex/introduction.tex <==
\section{Introduction}\label{sec:introduction}

Recently, channel state information~(CSI) of Wi-Fi signals has been increasingly exploited for person identification~\cite{xin2016freesense,zeng2016wiwho,zhang2016wifi,wang2016gait,shi2017smart,lv2017device,pokkunuru2018neuralwave} due to the pervasiveness and low cost in deployment. Besides, Wi-Fi based person identification enables passive identification, i.e., high user-friendly. What's more important, unlike popular face recognition systems being vulnerable to the replay attacks \cite{smith2015face}, or fingerprint recognition struggling for spoofing attacks from 3D printed models \cite{foolphone}, it is harder to fool the Wi-Fi based person identification system because the attack needs extremely vivid imitation on user behaviors.

Among previous work, CSI monitoring during user ambulation are the most prevailing CSI-based identification approaches ~\cite{xin2016freesense,zeng2016wiwho,zhang2016wifi,wang2016gait,lv2017device,pokkunuru2018neuralwave}, which demand users to walk along pre-defined paths and record corresponding Wi-Fi CSI series simultaneously. Then the recorded CSI is either to extract specific gait metric such as walking speed for identification~\cite{wang2016gait}, or directly to learn identity classifiers with machine learning algorithms, e.g., support vector machine~\cite{xin2016freesense,zeng2016wiwho,zhang2016wifi,lv2017device} or deep neural networks~\cite{pokkunuru2018neuralwave}. However, to recognize a person's gait, one must walk along the pre-defined paths again for several meters, e.g., 2-3m in \cite{zeng2016wiwho} and 5m in \cite{xin2016freesense}, which is labor intensive and time-consuming, thus largely limits use scenarios. To overcome limitations in gait-based approaches, Shi \textit{et al.}~\cite{shi2017smart} 
propose an activity-based person identification, which is built on the finding that CSI series corresponding to user daily activities like opening micro-oven carries identity-related patterns. Though the approach in \cite{shi2017smart} requires less labor work, daily activity patterns are inferior in robustness compared to gait.






\begin{figure}[t]
    \centering
    \includegraphics[width=0.47\linewidth]{figs/fig1_final.pdf}
    \includegraphics[width=0.5\linewidth]{figs/simple_mean.pdf}
    \caption{WiPIN rationale. When one stands in a Wi-Fi environment~(left), multi-path effect on the person body would lead to discriminated distortions in the Wi-Fi amplitude (right), which carries body information and can be well-designed for person identification.}
    \label{fig:first}
\vspace{-10pt}
\end{figure}
 

Retracing previous work, we conclude that Wi-Fi distortions caused by user behaviors, such as walking and other daily activities embedding behavior patterns, can be used for person identification. Moreover, we are wondering how CSI varies if a person does no operation just standing in a Wi-Fi environment. Fig.~\ref{fig:first} illustrates our preliminary experiment results for this wondering. We recruited 10 subjects to  stand in a same position, respectively, near the Wi-Fi transmitter and receiver~(left), meanwhile the corresponding CSI series are recorded. We average the CSI amplitudes over all recorded samples and plot them in the Fig.~\ref{fig:first}~(right). Majority of the amplitudes are discriminated, which demonstrates the potentiality for person identification.

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{figs/wipin_system.pdf}
    \caption{System framework. WiPIN is comprised of hardware and algorithms. The algorithms contain modules of signal pre-processing, data preparation, and identity matching. After deployed, WiPIN can identify legal users while reject illegal users. }
    \label{fig:system}
\end{figure*}

\begin{figure}[b]
    \centering
    \includegraphics[width=0.48\linewidth]{figs/fat.pdf}
    \includegraphics[width=0.48\linewidth]{figs/muscle.pdf}
    \caption{Information related to human body such as the fat rate and the muscle rate is embedded in the Wi-Fi distortion and can be well predicted by Wi-Fi signals with support vector regression~\cite{smola2004tutorial}.}
    \label{fig:fat}
\vspace{-5pt}
\end{figure}



We ascribe the reason of results shown in Fig.~\ref{fig:first} to that during the propagation, Wi-Fi signals must be embedded with certain information related to human body such as body shape, body fat rate, and body muscle rate, because of the multi-path effect on the body, and the absorption and reflection effect in the body. If this guess is correct, it is possible to perform person identification using Wi-Fi signals without any user activities like walking for several meters, but only standing for a second. To further confirm the guess, we measure the body fat rate and muscle rate of these subjects by a Mi$^\circledR$ body fat scale, then train a mapping function from CSI to aforesaid rates with support vector regression (SVR)~\cite{smola2004tutorial} (our not inferring body shape is because it is hard to get the ground-truth of body shape). Fig.~\ref{fig:fat} demonstrates that CSI distortions caused by standing persons are highly relevant with body fat rate and body muscle rate.




With the above analysis, we propose an operation-free passive person identification system, namely WiPIN. It can deeply extracts human body information from Wi-Fi distortion series caused by the user's presence, hence further identifies people with well-designed signal pre-processing and identity matching algorithms. One challenge in realizing the system is the mixture of body relevant signal and interference signals from multiple Wi-Fi propagation paths, and we tackle this problem by implementing a multi-path effect mitigation. Experimental results show that WiPIN achieves 92\% identification accuracy over 30 subjects with robustness to various experimental settings and low identifying time overhead, i.e., less than 300 ms. We summarize the main contributions of this paper as follows.

\begin{itemize}
    \item We propose WiPIN, a novel Wi-Fi signals-based passive person identification system, which has no requirement for the proactive user engagement in traditional identification systems, such as facing camera and scanning finger/iris. In addition, WiPIN is user-friendly and time-efficient in practice.
    
    \item We quantitatively study the rationale behind WiPIN, and conclude that during propagation, Wi-Fi signals are embedded with information related to human body. The intrinsic body information further used for person identification is robuster than behavior patterns. 
    
    \item WiPIN can classify authenticated users, as well as to reject illegal users that not seen before. We prototype WiPIN using commodity off-the-shelf Wi-Fi devices, and conduct extensive experiments to validate advances of WiPIN in various aspects including accuracy, robustness, time consumption, etc.   
    
\end{itemize}





